The photospheric energy and helicity budgets of the flux-injection hypothesis

The flux-injection hypothesis for driving coronal mass ejections (CMEs) requires the transport of substantial magnetic energy and helicity flux through the photosphere concomitant with the eruption. Under the magnetohydrodynamics approximation, these fluxes are produced by twisting magnetic field and/or flux emergence in the photosphere. A CME trajectory, observed 2000 September 12 and fitted with a flux-rope model constrains energy and helicity budgets for testing the flux-injection hypothesis. Optimal velocity profiles for several driving scenarios are estimated by minimizing the photospheric plasma velocities for a cylindrically symmetric flux-rope magnetic field subject to the flux budgets required by the flux-rope model. Ideal flux injection, involving only flux emergence, requires hypersonic upflows in excess of the solar escape velocity 617 km/s over an area of 6x10^8 km^2 to satisfy the energy and helicity budgets of the flux-rope model. These estimates are compared with magnetic field and Doppler measurements from Solar Heliospheric Observatory/Michelson Doppler Imager on 2000 September 12 at the footpoints of the CME. The observed Doppler signatures are insufficient to account for the required energy and helicity budgets of the flux-injection hypothesis.

==> dopmaps_VRO_all_all_table.tex <==
\newcommand{\chiall}{3898.0}
\newcommand{\dofall}{25455}
\begin{deluxetable}{ccccccccccccc}
\tabletypesize{\footnotesize}
\tablecaption{Fit-determined coefficients with $\chi^2=$\chiall~for disk-othonormalized
functions determined from 24 hours of MDI vector weighted
Dopplergams on 2003 September 12th.
\label{tab:limb_all}}
\tablehead{
\colhead{}&\multicolumn{3}{c}{$\mu$Rads/s}&
\colhead{\phantom{h}}&\multicolumn{8}{c}{m/s}\\
\cline{2-4}\cline{6-13}\\ 
\colhead{}&
\colhead{          $A_0$}  &
\colhead{          $A_2$}  &
\colhead{          $A_4$}  &
&
\colhead{          $L_0$}  &
\colhead{          $L_1$}  &
\colhead{          $L_2$}  &
\colhead{          $L_3$}  &
\colhead{          $L_4$}  &
\colhead{          $M_1$}  &
\colhead{          $M_2$}  &
\colhead{$H$}}
\startdata
$\widehat{\theta}$&
 3.1870  &
-0.1610  &
-0.0216  &
&
                                        131  &
                                        174  &
                                         88  &
                                         10  &
                                    \phs-3.1  &
                                    \phs-17.4  &
                                        0.6  &
                                        29.1 \\
$\widehat{\sigma}$&
                                    \phs 0.0021  &
                                    \phs 0.0027  &
                                    \phs 0.0027  &
&
                                         19  &
                                         26  &
                                         21  &
                                         11  &
                                    \phs 3.5  &
                                    \phs  3.0  &
                                        0.4  &
                                         5.0 \\
$\widehat{t}$&
 1496.81  &
  -59.19  &
   -8.05  &
&
    6.89  &
    6.64  &
    4.19  &
    0.92  &
   -0.88  &
   -5.76  &
    1.59  &
    5.87 \\
\%&
 0.0  &
 0.0  &
 0.0  &
&
 0.0  &
 0.0  &
 0.0  &
35.8  &
37.7  &
 0.0  &
11.1  &
 0.0 \\
\hline
$\widehat{\overline{\mu}}$&
                            \phn\phn\phn 3.1556  &
                                    \phs-0.1610  &
                                    \phs-0.0312  &
&
                                        127  &
                                        160  &
                                         88  &
                                         14  &
                                    \phs 2.0  &
                                    \phs  6.2  &
                                        0.1  &
                                         8.1 \\
$\widehat{\sigma}$&
                                    \phs 0.1366  &
                                    \phs 0.0238  &
                                    \phs 0.0136  &
&
                                        252  &
                                         29  &
                                         24  &
                                         12  &
                                    \phs 5.4  &
                                    \phs 36.0  &
                                        8.6  &
                                        77.1 \\
\hline
$\widehat{z}$&
   0.23  &
   0.00  &
   0.69  &
&
   0.02  &
   0.34  &
  -0.00  &
  -0.25  &
  -0.79  &
  -0.65  &
   0.06  &
   0.27 \\
\enddata
\end{deluxetable}


==> dopmaps_VRO_table.tex <==
\newcommand{\chisome}{3901.1}
\newcommand{\dofsome}{25457}
\begin{deluxetable*}{ccccccccccccc}
\renewcommand{\phs}{\phm{-}}
\tabletypesize{\footnotesize}
\tablecaption{\dopplercaption\label{tab:limb_all}}
\tablehead{
\colhead{}&\multicolumn{3}{c}{$\mu$Rads/s}&
\colhead{\phantom{h}}&\multicolumn{6}{c}{m/s}\\
\cline{2-4}\cline{6-11}
\colhead{\Top}&
\colhead{          $A_0$}  &
\colhead{          $A_2$}  &
\colhead{          $A_4$}  &
&
\colhead{          $L_0$}  &
\colhead{          $L_1$}  &
\colhead{          $L_2$}  &
\colhead{          $L_3$}  &
\colhead{          $M_1$}  &
\colhead{$H$}}
\startdata
$\widehat{\theta}$&
 3.1870  &
-0.1611  &
-0.0217  &
&
147  &
195  &
105  &
 20  &
-16.3  &
26.5 \\
$\widehat{\sigma}_\theta$&
                                         0.0021  &
                                    \phs 0.0027  &
                                    \phs 0.0027  &
&
                                \phn\phn  5  &
                                \phn\phn  7  &
                                \phn\phn  5  &
                                    \phn  2  &
                                \phs\phn  2.9  &
                                    \phn 4.7 \\
\noalign{\vskip0.05in}
$\widehat{t}_\theta$&
 1497.05  &
  -59.23  &
   -8.07  &
&
   25.72  &
   26.07  &
   19.49  &
    9.22  &
   -5.52  &
    5.63 \\
\%\Bot&
0.00  &
0.00  &
0.00  &
&
 0.0  &
 0.0  &
 0.0  &
 0.0  &
 0.0  &
 0.0 \\
\hline
$\widehat{\overline{\mu}}$\Top&
 3.1556  &
-0.1610  &
-0.0312  &
&
127  &
160  &
 88  &
 14  &
  6.2  &
 8.1 \\
$\widehat{\sigma}_{\overline{\mu}}$\Bot&
                                         0.1366  &
                                    \phs 0.0238  &
                                    \phs 0.0136  &
&
                                        252  &
                                    \phn 29  &
                                         24  &
                                         12  &
                                         36.0  &
                                        77.1 \\
\hline
$\widehat{t}_{\theta\overline{\mu}}$\Top&
   0.23  &
  -0.00  &
   0.69  &
&
   0.08  &
   1.16  &
   0.67  &
   0.45  &
  -0.62  &
   0.24 \\
\%&
  85.61  &
  99.78  &
  61.64  &
&
  94.97  &
  45.40  &
  62.22  &
  73.23  &
  64.57  &
  85.10 \\
\enddata
\end{deluxetable*}

